Security for Distributed Deep Neural Networks Towards Data Confidentiality & Intellectual Property Protection

Current developments in Enterprise Systems observe a paradigm shift, moving the needle from the backend to the edge sectors of those; by distributing data, decentralizing applications and integrating novel components seamlessly to the central systems. Distributively deployed AI capabilities will thrust this transition. Several non-functional requirements arise along with these developments, security being at the center of the discussions. Bearing those requirements in mind, hereby we propose an approach to holistically protect distributed Deep Neural Network (DNN) based/enhanced software assets, i.e. confidentiality of their input & output data streams as well as safeguarding their Intellectual Property. Making use of Fully Homomorphic Encryption (FHE), our approach enables the protection of Distributed Neural Networks, while processing encrypted data. On that respect we evaluate the feasibility of this solution on a Convolutional Neuronal Network (CNN) for image classification deployed on distributed infrastructures.

==> sections/Architecture.tex <==
\section{Architecture}
\label{sec:architecture}

In this section we outline the architecture of our IP protection system, as depicted in Figure \ref{fig:prDiag}.

\begin{figure}[ht]%
  \centering
	\includegraphics[width=0.5\textwidth]{images/procDiag2N.png}%
	\caption[ProcDiag]{Activity Diagram in our solution.}%
	\label{fig:prDiag}%
\end{figure}

\subsection{Encryption of trained DNN}
\label{subsection:encryptionoftraineddnn}
In the backend, a DNN is trained within a \textit{DNN Training Agent}, \circled{1}. The outcome of the training (NN architecture and parameters) is pushed to the \textit{Trained DNN Protection Agent}, \circled{3}. Alternatively, an already trained DNN can be imported directly into the \textit{Protection Agent}.
The \textit{DNN Protection Agent} generates a Fully Homomorphic key pair from the \textit{Key Generator} component, \circled{2}. The DNN is then encrypted and stored together with its homomorphic key pair in the \textit{Trained and Protected DNN Database}, \circled{4}.

\subsection{Deployment of trained and protected DNN}
\label{subsection:deploymentoftrainedandprotecteddnn}
At the deployment phase, the \textit{Trained DNN Deployment Agent} deploys the DNN on decentralized systems, together with its public key, \circled{5}.

\subsection{DNN processing}
\label{subsection:dnnprocessing}        
On the distributed system, data is collected by a \textit{Data Stream Acquisition} component, \circled{7}, and forwarded to the \textit{DNN Processing Agent}, \circled{6}. Input layer does not involve any computation, and therefore can be seamlessly FHE encrypted as follows

\begin{equation}
\mathbf{X} \xrightarrow{encryption} Enc_{\mathbf{pub}} (X) = \encr{X}
\end{equation}

Encrypted inferences are sent to the \textit{Decryption Agent}, \circled{8}, for their decryption using the private key associated to the DNN, \circled{9}. FHE encryption propagates across the DNN layers, from input to output layer.
By construction, output layer is encrypted homomorphically\todo{this is a weird paragraph}.

IP of the DNN, together with the computed inferences, is protected from any disclosure on the distributed system throughout the entire process.


The decryption of the last layer's output $\mathbf{Y}$ is done with the private encryption key \textit{priv}, as in standard asymmetric encryption schemes:

\begin{equation} \encr{\mathbf{A^{[L]}}} \xrightarrow{decryption} Dec_{\mathbf{priv}}\left(\encr{\mathbf{A^{[L]}}}\right) =\mathbf{Y}
\end{equation}




==> sections/ArchitectureEvaluation.tex <==
\section{Architecture \& Evaluation}
\label{sec:architectureandevaluation}

\subsection{Architecture}
\label{subsec:architecture}

In this section we outline the architecture of our IP protection system, as depicted in Figure \ref{fig:prDiag}.

\begin{figure}[ht]%
  \centering
	\includegraphics[width=0.48\textwidth]{images/procDiag2N.png}%
	\caption[ProcDiag]{Activity Diagram in our solution.}%
	\label{fig:prDiag}%
\end{figure}

\paragraph{Encryption of trained DNN}	\circled{1}	\circled{2} \circled{3} \circled{4}	\newline 	 
In the backend, a DNN is trained within a \textit{DNN Training Agent}. The outcome of the training (NN architecture and parameters) is pushed to the \textit{Trained DNN Protection Agent}. Alternatively, an already trained DNN can be imported directly into the \textit{Protection Agent}.

The \textit{DNN Protection Agent} generates a Fully Homomorphic key pair from the \textit{Key Generator} component. The DNN is then encrypted and stored together with its homomorphic key pair in the \textit{Trained and Protected DNN Database}.

\paragraph{Deployment of trained and protected DNN} 	\circled{5}	    \newline
At the deployment phase, the \textit{Trained DNN Deployment Agent} deploys the DNN on decentralized systems, together with its public key.

\paragraph{DNN processing}	\circled{6} \circled{7} \circled{8} \circled{9}		 \newline         
On the distributed system, data is collected by a \textit{Data Stream Acquisition} component, and forwarded to the \textit{DNN Processing Agent}. Encrypted inferences are sent to the \textit{Decryption Agent} for their decryption using the private key associated to the DNN.

IP of the DNN, together with the computed inferences, is protected from any disclosure on the distributed system throughout the entire process.

\newpage
\subsection{Evaluation}
\label{subsec:Evaluation}

\subsubsection{Setup}

\paragraph{Hardware}
\textcolor{red}{left open for the time being, depending on availability of JETSON TX2}
We demonstrate our approach on Keras CNN CIFRAS10 dataset, with an evaluation running on Jetson TX2 (GPU NVIDIA Pascal™, 256 CUDA cores, CPU HMP Dual Denver 2/2 MB L2 + Quad ARM® A57/2 MB L2, Memory 8 GB 128 bit LPDDR4 59.7 GB/s, Disk 32 GB eMMC, SDIO, SATA)

\subsubsection{Setup Software} 
\label{subsubsection:software}

\paragraph{FHE library}
We use SEAL\cite{sealcrypto} library from Microsoft Research for the evaluation of our approach.
Our choice was dictated by three the performance of this implementation, 
The choice for this library is motivated by the performance of the library, its support of novel schemes such as CKKS\ref{CKKS} \ref{SEAL2.3.1}. 


\paragraph{Model DNN}

As depicted in Figure \ref{fig:KerasCNN}, we use Keras Convolutional Neural Networks \cite{}.
Even though this implementation of CNN is not prone to be the most efficient compared to Yolo \cite{Yolo}, our choice was rather based on the accessibility of the model, and the ability to intercept layer, and encrypt them.

This is worth to mention that our approach is fully agnostic from NN topology, or implementation.
But for sake of simplicity of NN model modification, we choose Keras NN.

In order to conduct our experiment, we had to 
\begin{itemize}
\item{Train}
\item{Encrypt Model}
\item{Perform Encrypted Inference}
\item{Decrypt Inference}
\end{itemize}

\begin{figure}[ht]%
  \centering
	\includegraphics[width=0.2\textwidth]{images/KerasCNN.png}%
	\caption[KerasCNN]{Keras Convolutional Neural Network.}%
	\label{fig:KerasCNN}%
\end{figure}



\subsection{Evaluation}
\label{subsection:evaluation}


\paragraph{Activation Function Evaluation}
\label{subsec:activationfunctionevaluation}

As discussed in section \ref{}, FHE cannot operate on activation functions.
Due to its innate non-linearity, they need to be approximated with polynomials. (Gilad-Bachrach et al., 2016) proposed
using only s(z) approximating it with a square function. (Chabanne et al., 2017) used Taylor polynomials around x = 0, studying performance based on the polynomial degree. (Hesamifard et al., 2017) approximate instead the derivative of the function and then integrate to obtain their approximation. One alternative would be to use Chebyshev polynomials.

During our evaluation, we experiment ReLU function approximation as follows 
\begin{itemize}
\item{No Activation}
\item{Modified Softplus}
\item{Taylor Serie Approximation}
\end{itemize}

\begin{figure}[ht]%
  \centering
	\includegraphics[width=0.2\textwidth]{images/AccuracyApproximation.png}%
	\caption[ActivationFunctionApproximation]{Activation Function Evaluation.}%
	\label{fig:ActivationFunctionApproximation}%
\end{figure}

\begin{figure}[ht]%
  \centering
	\includegraphics[width=0.2\textwidth]{images/KerasCNN_NoActivation.png}%
	\caption[KerasCNNNoActivation]{Keras Convolutional Neural Network with No Activation Function for Classifier.}%
	\label{fig:KerasCNN_noactivation}%
\end{figure}

\begin{figure}[ht]%
  \centering
	\includegraphics[width=0.2\textwidth]{images/KerasCNN_SoftMaxPolyApproximation.png}%
	\caption[KerasCNNSoftplusApproximation]{Keras Convolutional Neural Network with Softplus Approximation.}%
	\label{fig:KerasCNN_softplus}%
\end{figure}

\begin{figure}[ht]%
  \centering
	\includegraphics[width=0.2\textwidth]{images/KerasCNN.png}%
	\caption[KerasCNN]{Keras Convolutional Neural Network.}%
	\label{fig:KerasCNN}%
\end{figure}

\paragraph{Evaluation}

Model Encryption - Done at backend level - no performance issue\\

Data Encryption & Processing Encryption\\

Processing Encryption Only - show number on performance computation memory disk usage accuracy loss\\
KERAS last layer
KERAS last layer + softplus function approximation
KERAS last layer + no activation function approximation

Decryption - done at the backend level - no performance issue there\\






==> sections/tabletest.tex <==

\begin{table*}[!ht]
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|}
\cline{2-10}
                                               & \multicolumn{9}{c|}{\textbf{Achieved Security Level (bits)}}                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \cline{2-10} 
                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{128}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{192}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{256}} & \multicolumn{1}{c|}{\textit{128}} & \multicolumn{1}{c|}{\textit{192}} & \multicolumn{1}{c|}{\textit{256}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{128}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{192}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{256}} \\ \hhline{~|---------|}%\cline{2-10} 
                                               & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textit{Full Classifier - Square Activation}}                                                                                                & \multicolumn{3}{c|}{\textit{Full Classifier - No Activation}}                                                    & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textit{Last Layer}}                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{Time to Compute}} & \cellcolor[HTML]{EFEFEF}2902.6s                           & \cellcolor[HTML]{EFEFEF}1048.6s                           & \cellcolor[HTML]{EFEFEF}5627.0s                           & 367.1s                            & 272.2s                            & 835.9s                            & \cellcolor[HTML]{EFEFEF}19.1s                             & \cellcolor[HTML]{EFEFEF}19.2s                             & \cellcolor[HTML]{EFEFEF}40.2s                             \\ \hline
\multicolumn{1}{|l|}{\textbf{Memory}}          & \cellcolor[HTML]{EFEFEF}5047.8Mb                          & \cellcolor[HTML]{EFEFEF}5809.4Mb                          & \cellcolor[HTML]{EFEFEF}4906.1Mb                          & 2314.8Mb                          & 1733.7Mb                          & 4644.5Mb                          & \cellcolor[HTML]{EFEFEF}119.5Mb                           & \cellcolor[HTML]{EFEFEF}118.5Mb                           & \cellcolor[HTML]{EFEFEF}252.8Mb                           \\ \hline
%\multicolumn{1}{|l|}{\textbf{Noise Budget}}    & \cellcolor[HTML]{EFEFEF}398.0                             & \cellcolor[HTML]{EFEFEF}260.0                             & \cellcolor[HTML]{EFEFEF}408.0                             & 187.0                             & 121.0                             & 187.0                             & \cellcolor[HTML]{EFEFEF}83.0                              & \cellcolor[HTML]{EFEFEF}49.0                              & \cellcolor[HTML]{EFEFEF}90.0                              \\ \hline
\multicolumn{1}{|l|}{\textbf{Remaining Noise}} & \cellcolor[HTML]{EFEFEF}206.0                             & \cellcolor[HTML]{EFEFEF}65.0                              & \cellcolor[HTML]{EFEFEF}76.0                              & 79.0                              & 11.0                              & 3.0                               & \cellcolor[HTML]{EFEFEF}45.0                              & \cellcolor[HTML]{EFEFEF}10.0                              & \cellcolor[HTML]{EFEFEF}52.0                              \\ \hline
\end{tabular}
\caption{hodor}
\label{tab:hodor}
\end{table*}

